Stabilizing Queuing Networks with Model Data-Independent Control

Classical queuing network control strategies typically rely on accurate knowledge of model data, i.e., arrival and service rates. However, such data are not always available and may be time-variant. To address this challenge, we consider a class of model data-independent (MDI) control policies that only rely on traffic state observation and network topology. Specifically, we focus on the MDI control policies that can stabilize multi-class Markovian queuing networks under centralized and decentralized policies. Control actions include routing, sequencing, and holding. By expanding the routes and constructing piecewise-linear test functions, we derive an easy-to-use criterion to check the stability of a multi-class network under a given MDI policy. For stabilizable multi-class networks, we show that a centralized, stabilizing MDI policy exists. For stabilizable single-class networks, we further show that a decentralized, stabilizing MDI policy exists. In addition, for both settings, we construct explicit policies that attain maximal throughput and present numerical examples to illustrate the results.

==> Texts/70_Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/photo_xq.jpg}}]{Qian Xie}
is a PhD student at the Department of Civil and Urban Engineering and the C2SMART University Transportation Center in the New York University Tandon School of Engineering.
She received her B.Eng. degree in Computer Science from Tsinghua University in 2019.
She is interested in studying resilience of civil infrastructures and designing secure network systems, using control-theoretic and game-theoretic approaches.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin}}]{Li Jin}
is Assistant Professor (2021--present) at the UM Joint Institute and the School of Electronic Information and Electrical Engineering, Shanghai Jiao Tong University, China. He is also Research Assistant Professor and was Assistant Professor (2018--2020) in the Tandon School of Engineering, New York University, USA. He received his B.Eng. from Shanghai Jiao Tong University in 2011, M.S. from Purdue University, USA in 2012, and Ph.D. from the Massachusetts Institute of Technology, USA in 2018. He was also a Visiting Scholar at the University of Erlangen-Nuremberg, Germany in 2016. His research uses ideas from stochastic processes, control, optimization, and machine learning to address key challenges in smart and connected systems. Specific applications include connected and autonomous vehicles, intelligent transportation systems, air traffic control, and smart pipeline transportation.
\end{IEEEbiography}
